Asynchronous Execution of Heterogeneous Tasks in ML-driven HPC Workflows

Heterogeneous scientific workflows consist of numerous types of tasks that require executing on heterogeneous resources. Asynchronous execution of those tasks is crucial to improve resource utilization, task throughput and reduce workflows' makespan. Therefore, middleware capable of scheduling and executing different task types across heterogeneous resources must enable asynchronous execution of tasks. In this paper, we investigate the requirements and properties of the asynchronous task execution of machine learning (ML)-driven high performance computing (HPC) workflows. We model the degree of asynchronicity permitted for arbitrary workflows and propose key metrics that can be used to determine qualitative benefits when employing asynchronous execution. Our experiments represent relevant scientific drivers, we perform them at scale on Summit, and we show that the performance enhancements due to asynchronous execution are consistent with our model.

==> intro.tex <==
%!TEX root = main.tex

The coupling of high performance computing (HPC) capabilities, artificial
intelligence (AI) and machine learning (ML) has been accelerating scientific
research and discovery across domains~\cite{}. \ldots

\ldots

Many scientific HPC workflows consist of computational pipelines that support
the execution of heterogeneous tasks at large scale. Those tasks have diverse
dimensions of heterogeneity: implementation, e.g., executables or
function/methods in an arbitrary language;  resource requirements, e.g.,
executing on CPUs and/or GPUs, computational or data intensive operations;
duration, from less than a second to many hours; size, from a core to many cores
over one or more compute nodes; and scientific objective, e.g., simulating
physical systems, training models, aggregating data and so on.

Executing heterogeneous scientific workflows poses several challenges. In this
paper, we focus on the resource management challenge that stems from having to
execute possibly related tasks with diverse resource requirements. Consider
having to execute both simulations tasks, each requiring few nodes of an high
performance computing (HPC) machine, and machine learning (ML) tasks, each
requiring one GPU of a single node.

Historically, the simulation tasks would generate data and the ML tasks would
use that data for training or inference. However, as continuous training,
surrogate re-training and optimal execution of campaigns become increasingly
important, the hard temporal separation of simulations and ML is no longer
tenable. Further, simulation tasks feed data to the ML tasks, creating a
dependence between the two types of task. A naive approach in which all the
simulations run before the ML code leads to poor resource utilization: while
the ML tasks run, a large amount of the allocated HPC resource idles.

Asynchronous execution is a design approach that can improve resource
utilization when executing heterogeneous workflows on HPC resources. In that
approach, different types of task are independently executed so as to
concurrently utilize the available resources. Following the previous example, in
a asynchronous execution, both simulation and ML tasks execute independently and
concurrently, eventually increasing overall resource utilization. Applicability
of asynchronous execution depends on the specifics of each workflow, and
requires dedicated data and control flows design. As such, understanding the
extent to which asynchronous execution can be utilized for a given workflow and
quantifying the performance benefits that could be achieved by implementing an
asynchronous execution, are determining factors in the design of an HPC
scientific workflow.

In this paper, we provide the necessary and sufficient conditions for a general
workflow to achieve asynchrony,  model asynchronous execution and offer an
experimental characterization of the improvements it can bring in terms of
resource utilization and task throughput. Given a specific set of workflow
requirements, both model and characterization are tools that workflow
application developers can use to asses the benefits that this approach could
bring. We offer four main contributions: (1) an asynchronous implementation of
DeepDriveMD (DDMD), our framework to execute ML-driven molecular-dynamics
workflows on HPC platforms at scale; (2) a performance evaluation of
asynchronous DDMD with a ML-driven simulation workflow; (3) a model of
asynchronous behavior; and (4) a general performance evaluation of that model
for workflows with a varying degree of asynchronous execution.

\S\ref{sec:usecase} we introduce IMPECCABLE, explaining how it is a paradigmatic
use case for asynchronous execution. In \S\ref{sec:design}, we define
asynchronous execution and its relationship with data and control flow when
designing a workflow application. In \S\ref{sec:experiments} we formalize the
notion of asynchronous execution by modeling its behavior and performance for
the metrics of task throughput and resource utilization. In \S\ref{sec:perf} we
compare synchronous and asynchronous execution of IMPECCABLE, measuring the
benefits of the latter. We then generalize those results, offering an
experimental characterization of the performance gains provided by different
degrees of heterogeneity for a given workflow. Finally, in
\S\ref{sec:conclusions} we discuss the implications of our model and performance
analysis for the design of workflow applications with heterogeneous tasks, when
executed on HPC resources at scale.

% This paper offers three main contributions: an analysis of the design required
% by IMPECCABLE to perform adaptive runtime execution of tasks with diverse
% dimensions of heterogeneity; a performance characterization of the proposed
% design, based on workload based on a statistical parameterization of IMPECCABLE
% workflows' requirements; and a quantifications of the benefits obtained by an
% asynchronous execution of IMPECCABLE workflows, compared to their synchronous
% execution. Together, those contribution will drive the development of IMPECCABLE
% and all the workflows and pipelines with the same computational characteristics.
% The experimental results of this paper will allow to ground their design on
% quantifiable performance gains.

% In the next section we briefly introduce IMPECCABLE use case and show how it is
% consistent with a class of workflows in which machine learning (ML) is used to
% drive physical simulations, improving scientific and computational efficiencies.
% We describe different types of task heterogeneity that characterize those
% workflows, showing how they depend on runtime adaptive capabilities for their
% execution. In \S\ref{sec:design}, we propose a design for IMPECCABLE in which
% heterogeneous tasks execute asynchronously and exchange data, and adaptivity
% enable varying the ration among task types at runtime, depending on the results
% of ongoing computations. In \S\ref{sec:perf} we introduce our experimental
% design, and evaluate the results of running those experiments to characterize
% the performance of our design based on IMPECCABLE workflows' requirements. We
% close the paper with a brief review of related work (\S\ref{sec:related}) and
% some conclusions (\S\ref{sec:conclusions}.)

% Executing heterogeneous scientific workflows poses several challenges. Among
% those, three are particularly relevant when considering middleware development:
% effective and efficient concurrent execution of heterogenous tasks on
% heterogeneous resources; adoption of methodologies to optimize execution at
% runtime; coordinating the execution of those diverse workflows at scale on
% possibly leadership-class HPC platforms.


==> motivation_old.tex <==
%!TEX root = main.tex

We argue there exist two conditions for workflow-level asynchronicity (WLA): (1)
inter-task dependencies and (2) resource availability. As detailed below, these
conditions, in addition to task execution time (TX), dictate resource
utilization and task throughput, two key metrics that determine the total time
to execution (TTX, or makespan) when employing asynchronous task execution. The
importance of considering only executing and not running tasks must be stressed
as a running task will increase resource utilization but will not progress a
workflow to completion.

\subsection{Condition I: Inter-Task Dependencies}
\label{ssec:cond-dependencies}

% \TODO{
In this paper, we mention asynchronous execution of workflow's heterogeneous
tasks where there are no dependencies among the given tasks. We focus on data
dependencies because, as seen in \S\ref{sec:related}, we assume tasks to be
black boxes. Consistent with common practice, we represent a workflow dependency
graph (DG) as a directed acyclic graph (DAG), where edges are data dependencies
and nodes are tasks. Asynchronous task execution only applies to workflows that
contain one or more forks with diverging paths. As such, given enough resources,
independent tasks of different types can execute asynchronously.

\ozgurnote{For a task, black box means that we do not see inner works of the
task, which include the inter-task communication however we can see data
produced or used by the given task.} \mtnote{Maybe explain the relation between
data dependences and black boxes a bit more in detail? It might not be
immediately evident to the reader.} \ozgurnote{I agree but it seems like we
already mentioned briefly in Related work as --- We assume tasks to be black
boxes and therefore, in our modeling, we abstract away the details of
asynchronous communication as data dependencies are assumed to be satisfied,
either before or during execution ---}\mtnote{OK, proposed an explicit reference
in the text. If it works for you, feel free to comment out these thread.}
\ozgurnote{}

% }
%\FIXME{Question: can we eliminate  "that do not eventually converge" because
% while whole WLA depends on that in a given time it only depends on possible
% dependencies between executing tasks}\mtnote{Done.} \DELETE{When representing
% a workflow as a directed acyclic graph (DAG), asynchronous task execution only
% applies to workflows which contain one or more forks with diverging paths that
% do not eventually converge. As such, given enough resources, independent tasks
% of different types can execute concurrently.}

% \TODO{
Figure~\ref{fig:dags} shows four DGs representatives of four workflows with
varying levels of inter-task dependence. Note that task set indices are ordered
breadth-first, and that the y-axis of our DG does not correlate with time. We
define the degree of asynchronicity ($\doadep$) as the number of independent
execution branches minus 1.
% \TODO{
To discover independent branches we perform a Depth Fist Search (DFS) on the DG.
% }
%\ozgurnote{Add some explanations w.r.t. how we traverse the graph.}
The lower bound on  ($\doadep$), permitted by task dependencies, arises when the
DG is sequential, \eg, a linear chain, Fig.~\ref{sfig:graph-chain} for which
$\doadep = 0$. The upper bound, \ie, completely asynchronous, arises a DG whose
edge set is the empty set such as that in Fig.~\ref{sfig:graph-indep}, where
$\doadep = n$. In between these bounds, asynchronicity in general varies as a
function of the number of forks with diverging paths that do not rejoin.

% }
% \DELETE{Representing a workflow as a DAG allows one to visualize dependencies
% (edges) between tasks (nodes). Figure~\ref{fig:dags} shows four DAGs
% representative of four distinct workflows with various levels of inter-task
% dependence. Task set indices are ordered breadth-first. The lower bound on the
% degree of asynchronicity ($\doadep$), permitted by task dependencies, arises
% when the DAG is sequential, \eg, a linear chain, Fig.~\ref{sfig:graph-chain}
% for which $\doadep = 0$. The upper bound, \ie, completely asynchronous, arises
% a DAG whose edge set is the empty set such as that in
% Fig.~\ref{sfig:graph-indep} where $\doadep = n$. In between these bounds,
% asynchronicity in general varies as a function of the number of forks with
% diverging paths that do not rejoin.}
%
%\begin{figure}[!ht] \centering \begin{subfigure}[b]{0.65\columnwidth}
%     \centering
%     {\raisebox{45pt}{\includegraphics[width=\columnwidth]{fig/graph-chain.pdf}}}
%     \caption{$\doadep = 0$} \label{sfig:graph-chain} \end{subfigure}% \hfill
%     \begin{subfigure}[b]{0.35\columnwidth} \centering
%     \includegraphics[width=\columnwidth]{fig/graph-doa1.pdf} \caption{$\doadep
%     = 1$} \label{sfig:graph-doa1} \end{subfigure} \\
%     \begin{subfigure}[b]{0.52\columnwidth} \centering
%         \includegraphics[width=\columnwidth]{fig/graph-doa4.pdf}
%         \caption{$\doadep = 4$} \label{sfig:graph-doa4} \end{subfigure}%
%         \hfill \begin{subfigure}[b]{0.48\columnwidth} \centering
%         {\raisebox{18pt}{\includegraphics[width=\columnwidth]{fig/indep-graph.pdf}}}
%         \caption{$\doadep = n$} \label{sfig:graph-indep} \end{subfigure}
%         \caption{Abstract dependency graphs and their respective task
%         dependency degree of asynchrony, $\doadep$. These are abstract in the
%         sense that only task sets (nodes), their orderings (indices) and
%         dependencies (edges) are given. These DGs contain no information about
%         the number of tasks in each task set, their resource requirements,
%         task execution time (TX), \etc~Task set indices are ordered in a
%         breadth-first manner.} \label{fig:dags} \end{figure}


\begin{figure}[!ht]
     \centering
     \begin{subfigure}[b]{0.25\columnwidth}
         \centering
         {\raisebox{30pt}{\includegraphics[width=\columnwidth]{fig/graph-chain.pdf}}}
         \caption{$\doadep = 0$}
         \label{sfig:graph-chain}
     \end{subfigure}%
     \hfill
     \begin{subfigure}[b]{0.19\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{fig/graph-doa1.pdf}
         \caption{$\doadep = 1$}
         \label{sfig:graph-doa1}
     \end{subfigure} %
     \hfill
     \begin{subfigure}[b]{0.30\columnwidth}
         \centering
         {\raisebox{15pt}{\includegraphics[width=\columnwidth]{fig/graph-doa4.pdf}}}
         \caption{$\doadep = 4$}
         \label{sfig:graph-doa4}
     \end{subfigure}%
     \hfill
     \begin{subfigure}[b]{0.25\columnwidth}
         \centering
         {\raisebox{30pt}{\includegraphics[width=\columnwidth]{fig/indep-graph.pdf}}}
         \caption{$\doadep = n$}
         \label{sfig:graph-indep}
     \end{subfigure}
        \caption{Abstract dependency graphs and their respective task
        dependency degree of asynchrony, $\doadep$. These are abstract in the
        sense that only task sets (nodes), their orderings (indices) and
        dependencies (edges) are given. These DGs contain no information about
        the number of tasks in each task set, their resource requirements, task
        execution time (TX), \etc~Task set indices are ordered in a
        breadth-first manner.
        \ozgurnote{ testing if figure would look better side by side it is currently too big}
        }
        \label{fig:dags}
\end{figure}

\subsection{Condition II: Resource Availability}
\label{ssec:cond-resreqs}

Assuming unlimited resources, inter-task dependency is, in principle, the
condition for determining the degree of asynchronicity for a given
workflow. For example, the DAG in Fig.~\ref{sfig:graph-indep} has $\doadep = n$,
so in the case of infinite resources, each of the $n+1$ task sets' tasks can
execute asynchronously. In practice, however, resources are limited, and
therefore an additional condition based on the available (allocated) resources
must be imposed.

To describe the resource-permitted degree of asynchronicity, $\doares$, consider
again the workflow DG in Fig.~\ref{sfig:graph-indep}. Let $\widetilde{R}$ be
the set of all allocated resources and $\cup_i R_i$ be the set resources
required to asynchronously execute the $n+1$ task sets.
Complete asynchronicity is achieved if and only if $\cup_i R_i \subseteq
\widetilde{R}$, in which case $\doares >= \doadep = n$. On the other extreme, if
$R_i = \widetilde{R}~\forall_i$, then we have two possibilities: (1) execute each
task set in arbitrarily or based on a given scheduler's heuristics (since the
execution of the full set of tasks from any task set requires 100\% of the
allocated resources); or (2) execute from two or more task sets the subsets such
that $\cap_i R_i = \widetilde{R}$. Despite $\doares = 0$ in the first case and
$\doares > 0$ in the second, there exists an equivalence between the two wherein
the latter effectively is the collapse of a dependency-free DAG to a chain as in
Fig.~\ref{sfig:graph-chain}. This scenario highlights how haphazard attempts to
adopt asynchronicity into a workflow will not always yield any benefit for the
workflow as a whole, and instead can lead to significant loss of development
time during the design process.

Richer, albeit more complex, situations lie between the two extremes. Take, for
example, the workflow DAG of Fig.~\ref{sfig:graph-doa4}, which has $\doadep =
4$. Depending on the resource requirements for each of $T_2-T_9$ task sets, $0
\leq \doares \leq 5$. As such, we define,
%
\begin{equation}
    \text{WLA} \equiv \min[\doadep, \doares]
\end{equation}
%
to quantify the asynchronicity permitted by the workflow.
% \TODO{

%Note that asynchronous execution here implies concurrency but that not all
%concurrent executions are also asynchronous. Tasks can concurrently execute
%synchronously,
%\ie, when their execution depends on  explicit coordination at runtime.
%\ozgurnote{Adding your suggestion: \eg, when two tasks run by a single
%thread, they can created to run concurrently but they are synchronous if, for
%example, $task_2$ has to wait a package from $task_1$ to do some computation. On
%the other hand, some sequential execution (as oppose to concurrent) can be
%asynchronous, \ie, one does not have to wait for the other to complete to
%start/stop. \eg, assuming running one data generation task every 1 second, they
%are asynchronous when $task_i$ can start independent of the state of
%$task_{i-1}$ ---started, completed, running ---; however, they are synchronous
%when $task_i$ has to wait for $task_{i-1}$ to finish to start. }
%\mtnote{Proposing an iteration of the whole paragraph, please edit/discard as
%you see it fit: ``
Note that asynchronous executions are not necessarily concurrent, and
synchronous executions are not necessarily sequential. Tasks are asynchronous
when they can execute independently of one another, while tasks are concurrent
when they execute at the same time. Thus, asynchronous executions can be both
sequential or concurrent, depending on resource availability. For example, two
independent tasks (${T_O}$ and ${T_1}$ from fig \ref{sfig:graph-doa4}) can be
run one after the other if not enough resources are available to execute them
concurrently. Analogously, two tasks that depend on each other (\eg inter-task
communication dependency) can execute concurrently when enough resources are
available.
%''}


%\mtnote{Maybe give more details about the last sentence, after the `i.e.' so
%that the reader can `visualize' what that means? I also see the inverse, in
%which some sequential execution (as oppose to concurrent) can be asynchronous,
%as for example when two tasks are run within a single thread by the OS, but one
%does not depend on the other, i.e., one does not have to wait for the other to
%complete to start/stop. E.g., given 3 tasks and 1 thread, they are synchronous
%when 2 as to wait for 1 to finish to start; asynchronous when 2 can start
%independent of the state of 1---1 has started, 1 has completed, 1 is still
%running.}
% }
%
\subsection{Task Execution Time and Masking \FIXME{Is this a condition. I think it is more of a results I suggest we add a new section for this as benefits of WLA}}
\label{ssec:cond-ttx}

\mtnote{I think the flow might be: 1. we (formally?) define asynchronous
execution of heterogeneous workflow's tasks; 2. Once we know what asynchronous
execution is, we (formally?) explore the effects that asynchronous execution has
on commonly used metrics of workflow execution efficiency, i.e., makespan and
resource utilization; 3. We show that those effects depend on task and graph
properties, i.e., asynchronicy alone is not guarantee of better resource
utilization and/or makespan.} \ozgurnote{That sounds good to me I will try a
complete rewrite of theis entire section  with your suggestion as next section.
We can decide which one to keep}
\ozgurnote{}

A primary motivation for asynchronous task execution is to improve resource
utilization which, in turn, directly correlates with task throughput. However,
examples have already been given that show how the introduction of
asynchronicity does not guarantee increased task throughput, specifically when
the majority of upstream tasks (ancestors) dominate resource use. When a
workflow requires resources with a $\doares > 0$ and it is possible to exploit
TX \mtnote{what does it mean to `exploit TX'? Is this a reference to masking? If
so, should we explain masking before?}, the overall workflow TTX can be reduced
by achieving higher task throughput.

Leveraging TX can afford \textit{masking}, a technique wherein longer running
tasks effectively `hide' contributions from shorter running tasks' a workflow's
TTX. To illustrate masking, consider the workflow DG of
Fig.~\ref{sfig:graph-doa1} for which $\doadep = 1$. Assume the allocated
resources are such that once $T_0$ completes, the chains $\{T_1, T_3, T_5\}$ and
$\{T_2, T_4\}$ can execute asynchronously; then $\doares = \doadep = 1$. For
concreteness, further assume the following TTX assignments:
\begin{equation*}
    t_0 = 500\text{s},~t_1 = t_2 = 1000\text{s},~2t_3 = 2t_5 = t_4 = 4000\text{s}.
\end{equation*}

To demonstrate the utility of masking, we begin with a purely sequential
workflow using the Pipeline/Stage/Task (PST)
model~\cite{balasubramanian2018harnessing}, where the DG represents a pipeline,
each rank corresponds to a stage, and each task set to tasks. In the sequential
model, the TTX is given by,
%
%\begin{align}
\begin{equation}
    \tseq = \sum_i t_i + C, \label{eqn:tseq}
\end{equation}
%\end{align}
%
% \TODO{
where $i$ represents $i$th stage and $t$ represents TX of given stage,
% }
and $C$ is a constant representing the workflow management system's overheads
such as communications. In general, $C$ is negligible with task execution times
$O(10)$ minutes and larger. As such, we disregard small overheads in future
calculations but consider them in later analyses. Plugging into
Eqn.~\ref{eqn:tseq} the above assigned TX values, the sequential TTX is
$t^{\text{Seq}} = 7500\text{s}$.

We now demonstrate how the workflow TTX can be significantly reduced by
exploiting the conditions for asynchronicity and the parameters of the workflow;
specifically here, $\text{WLA} = \min(\doadep, \doares) = 1$ and the TX
assignments
% \TODO{
are the same as above.
% }.
First, the WLA enables asynchronous execution of the chains $H_1 \equiv \{T_1,
T_3, T_5\}$ and $H_2 \equiv \{T_2, T_4\}$. Second, the TX assignments lead to
masking such that the contribution from task set $T_5$ to the workflow TTX is
hidden by the execution of task set $T_4$ since $t_4 = t_3 + t_5$ and the
corresponding task sets now execute asynchronously. In general, the asynchronous
TTX for an asynchronous workflow is given by,
%
% \FIXME{OLD one to delete}
% \begin{align}
%     \label{eqn:tasync}
%     \tasync &= \sum_{i < j} t_i + \max[t_{H_j}]  \\
%             &\leq \tseq, \nonumber
% \end{align}
%
% \FIXME{New one}
\begin{align}
% \begin{equation}
    \label{eqn:tasync}
    \tasync &= \sum_{i} t_i + \max[tt_{H_j}] + C \\
            &\leq \tseq, \nonumber
% \end{equation}
\end{align}
%
% \TODO{
where $t_i$ represents the sequential task sets and $tt_{H_j}$ represents the
TTX of each independent branch.
% }
\begin{align}
%\begin{equation}
    \label{eqn:tth}
    tt_{H_j}&= \sum_{j} t_j  \\
            &\leq \tseq, \nonumber
%\end{equation}
\end{align}
%
% \DELETE{where the sum is over the sequential task sets and $j$ corresponds to
% the task set with the smallest index within the rank where one more
% asynchronicity-permitting forks occur (in this case, $j=1$).
% }
We have equality if and only if $t_{H_j} = t_{H_k}~\forall_{j,k}$. Asynchronous
execution of the workflow under discussion therefore has a TTX of $t_0 + t_{H_1}
= 5500\text{s}$. We define the relative improvement as,
%
\begin{align}
%\begin{equation}
    I &\equiv 1 - \frac{\tasync}{\tseq},
    \label{eqn:relimp}
%\end{equation}
\end{align}
%
for which, in this example, gives roughly a 26\% reduction compared to the
sequential execution. This example makes clear the potential gains when a
workflow is designed to leverage WLA as well as TX masking.



\ozgurnote{Parts I deleted from main. I think it is same with the text above this line.}
\section{Conditions and Motivations for Workflow-Level Asynchronicity}
\label{sec:conds}

We argue there exist two conditions for workflow-level asynchronicity (WLA): (1)
inter-task dependencies and (2) resource availability. As detailed below, these
conditions, in addition to task execution time (TX), dictate resource
utilization and task throughput, two key metrics that determine the total time
to execution (TTX, or makespan) when employing asynchronous task execution. The
importance of considering only executing and not running tasks must be stressed
as a running task will increase resource utilization but will not progress a
workflow to completion.

\subsection{Condition I: Inter-Task Dependencies}
\label{ssec:cond-dependencies}

% \TODO{
In this paper, we mention asynchronous execution of heterogeneous tasks where
there are no dependencies among the given tasks. We focus on data dependencies
because, as seen in \S\ref{sec:related}, we assume tasks to be black boxes.
\ozgurnote{For a task, black box means that we do not see inner works of the task,
which include the inter-task communication however we can see data produced or used by the given task.}
\mtnote{Maybe explain the relation between data dependences and black boxes a
bit more in detail? It might not be immediately evident to the reader.}
\ozgurnote{I agree but it seems like we already mentioned briefly in Related
work as --- We assume tasks to be black boxes and therefore, in our modeling, we
abstract away the details of asynchronous communication as data dependencies are
assumed to be satisfied, either before or during execution ---}\mtnote{OK,
proposed an explicit reference in the text. If it works for you, feel free to
comment out these thread.}
\ozgurnote{}
% For a better visualization
Consistent with common practice, we represent a workflow dependency graph (DG)
as a directed acyclic graph (DAG), where edges are data dependencies and nodes
are tasks. Asynchronous task execution only applies to workflows that contain
one or more forks with diverging paths.
% that do not eventually converge.
As such, given enough resources, independent tasks of different types can
execute asynchronously.

% }
%\FIXME{Question: can we eliminate  "that do not eventually converge" because
% while whole WLA depends on that in a given time it only depends on possible
% dependencies between executing tasks}\mtnote{Done.} \DELETE{When representing
% a workflow as a directed acyclic graph (DAG), asynchronous task execution only
% applies to workflows which contain one or more forks with diverging paths that
% do not eventually converge. As such, given enough resources, independent tasks
% of different types can execute concurrently.}

% \TODO{
Figure~\ref{fig:dags} shows four DGs representatives of four distinct workflows
with varying levels of inter-task dependence. Note that task set indices are
ordered breadth-first, and that the y-axis of our DG does not correlate with
time. We define the degree of asynchronicity ($\doadep$) as the number of
independent execution branches minus 1.
% \TODO{
To discover independent branches we perform a Depth Fist Search (DFS) on the DG.
% }
%\ozgurnote{Add some explanations w.r.t. how we traverse the graph.}
The lower bound on  ($\doadep$), permitted by task dependencies, arises when the
DG is sequential, \eg, a linear chain, Fig.~\ref{sfig:graph-chain} for which
$\doadep = 0$. The upper bound, \ie, completely asynchronous, arises a DG whose
edge set is the empty set such as that in Fig.~\ref{sfig:graph-indep}, where
$\doadep = n$. In between these bounds, asynchronicity in general varies as a
function of the number of forks with diverging paths that do not rejoin.

% }
% \DELETE{Representing a workflow as a DAG allows one to visualize dependencies (edges)
% between tasks (nodes). Figure~\ref{fig:dags} shows four DAGs representative of
% four distinct workflows with various levels of inter-task dependence. Task set
% indices are ordered breadth-first. The lower bound on the degree of
% asynchronicity ($\doadep$), permitted by task dependencies, arises when the DAG
% is sequential, \eg, a linear chain, Fig.~\ref{sfig:graph-chain} for which
% $\doadep = 0$. The upper bound, \ie, completely asynchronous, arises a DAG whose
% edge set is the empty set such as that in Fig.~\ref{sfig:graph-indep} where
% $\doadep = n$. In between these bounds, asynchronicity in general varies as a
% function of the number of forks with diverging paths that do not rejoin.}
%
%\begin{figure}[!ht]
%     \centering
%     \begin{subfigure}[b]{0.65\columnwidth}
%         \centering
%         {\raisebox{45pt}{\includegraphics[width=\columnwidth]{fig/graph-chain.pdf}}}
%         \caption{$\doadep = 0$}
%         \label{sfig:graph-chain}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}[b]{0.35\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{fig/graph-doa1.pdf}
%         \caption{$\doadep = 1$}
%         \label{sfig:graph-doa1}
%     \end{subfigure} \\
%     \begin{subfigure}[b]{0.52\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{fig/graph-doa4.pdf}
%         \caption{$\doadep = 4$}
%         \label{sfig:graph-doa4}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}[b]{0.48\columnwidth}
%         \centering
%         {\raisebox{18pt}{\includegraphics[width=\columnwidth]{fig/indep-graph.pdf}}}
%         \caption{$\doadep = n$}
%         \label{sfig:graph-indep}
%     \end{subfigure}
%        \caption{Abstract dependency graphs and their respective task
%        dependency degree of asynchrony, $\doadep$. These are abstract in the
%        sense that only task sets (nodes), their orderings (indices) and
%        dependencies (edges) are given. These DGs contain no information about
%        the number of tasks in each task set, their resource requirements, task
%        execution time (TX), \etc~Task set indices are ordered in a
%        breadth-first manner.}
%        \label{fig:dags}
%\end{figure}


\begin{figure}[!ht]
     \centering
     \begin{subfigure}[b]{0.25\columnwidth}
         \centering
         {\raisebox{30pt}{\includegraphics[width=\columnwidth]{fig/graph-chain.pdf}}}
         \caption{$\doadep = 0$}
         \label{sfig:graph-chain}
     \end{subfigure}%
     \hfill
     \begin{subfigure}[b]{0.19\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{fig/graph-doa1.pdf}
         \caption{$\doadep = 1$}
         \label{sfig:graph-doa1}
     \end{subfigure} %
     \hfill
     \begin{subfigure}[b]{0.30\columnwidth}
         \centering
         {\raisebox{15pt}{\includegraphics[width=\columnwidth]{fig/graph-doa4.pdf}}}
         \caption{$\doadep = 4$}
         \label{sfig:graph-doa4}
     \end{subfigure}%
     \hfill
     \begin{subfigure}[b]{0.25\columnwidth}
         \centering
         {\raisebox{30pt}{\includegraphics[width=\columnwidth]{fig/indep-graph.pdf}}}
         \caption{$\doadep = n$}
         \label{sfig:graph-indep}
     \end{subfigure}
        \caption{Abstract dependency graphs and their respective task
        dependency degree of asynchrony, $\doadep$. These are abstract in the
        sense that only task sets (nodes), their orderings (indices) and
        dependencies (edges) are given. These DGs contain no information about
        the number of tasks in each task set, their resource requirements, task
        execution time (TX), \etc~Task set indices are ordered in a
        breadth-first manner.
        \ozgurnote{ testing if figure would look better side by side it is currently too big}
        }
        \label{fig:dags}
\end{figure}

\subsection{Condition II: Resource Availability}
\label{ssec:cond-resreqs}

Assuming unlimited resources, inter-task dependency is, in principle, the
condition for determining the degree of asynchronicity for a given
workflow. For example, the DAG in Fig.~\ref{sfig:graph-indep} has $\doadep = n$,
so in the case of infinite resources, each of the $n+1$ task sets' tasks can
execute asynchronously. In practice, however, resources are limited, and
therefore an additional condition based on the available (allocated) resources
must be imposed.

To describe the resource-permitted degree of asynchronicity, $\doares$, consider
again the workflow DG in Fig.~\ref{sfig:graph-indep}. Let $\widetilde{R}$ be
the set of all allocated resources and $\cup_i R_i$ be the set resources
required to asynchronously execute the $n+1$ task sets.
Complete asynchronicity is achieved if and only if $\cup_i R_i \subseteq
\widetilde{R}$, in which case $\doares >= \doadep = n$. On the other extreme, if
$R_i = \widetilde{R}~\forall_i$, then we have two possibilities: (1) execute each
task set in arbitrarily or based on a given scheduler's heuristics (since the
execution of the full set of tasks from any task set requires 100\% of the
allocated resources); or (2) execute from two or more task sets the subsets such
that $\cap_i R_i = \widetilde{R}$. Despite $\doares = 0$ in the first case and
$\doares > 0$ in the second, there exists an equivalence between the two wherein
the latter effectively is the collapse of a dependency-free DAG to a chain as in
Fig.~\ref{sfig:graph-chain}. This scenario highlights how haphazard attempts to
adopt asynchronicity into a workflow will not always yield any benefit for the
workflow as a whole, and instead can lead to significant loss of development
time during the design process.

Richer, albeit more complex, situations lie between the two extremes. Take, for
example, the workflow DAG of Fig.~\ref{sfig:graph-doa4}, which has $\doadep =
4$. Depending on the resource requirements for each of $T_2-T_9$ task sets, $0
\leq \doares \leq 5$. As such, we define,
%
\begin{equation}
    \text{WLA} \equiv \min[\doadep, \doares]
\end{equation}
%
to quantify the asynchronicity permitted by the workflow.
% \TODO{

%Note that asynchronous execution here implies concurrency but that not all
%concurrent executions are also asynchronous. Tasks can concurrently execute
%synchronously,
%\ie, when their execution depends on  explicit coordination at runtime.
%\ozgurnote{Adding your suggestion: \eg, when two tasks run by a single
%thread, they can created to run concurrently but they are synchronous if, for
%example, $task_2$ has to wait a package from $task_1$ to do some computation. On
%the other hand, some sequential execution (as oppose to concurrent) can be
%asynchronous, \ie, one does not have to wait for the other to complete to
%start/stop. \eg, assuming running one data generation task every 1 second, they
%are asynchronous when $task_i$ can start independent of the state of
%$task_{i-1}$ ---started, completed, running ---; however, they are synchronous
%when $task_i$ has to wait for $task_{i-1}$ to finish to start. }
%\mtnote{Proposing an iteration of the whole paragraph, please edit/discard as
%you see it fit: ``
Note that asynchronous executions are not necessarily concurrent,
and synchronous executions are not necessarily sequential.
Tasks are asynchronous when they can execute independently of one another,
while tasks are concurrent when they execute at the same time.
Thus, asynchronous executions can be both sequential or concurrent,
depending on resource availability.
For example, two independent tasks
(${T_O}$ and ${T_1}$ from fig \ref{sfig:graph-doa4})
can be run one after the other if not enough resources are available to execute them concurrently.
Analogously, two tasks that depend on each other
(\eg inter-task communication dependency)
can execute concurrently when enough resources are available.
%''}


%\mtnote{Maybe give more details about the last sentence, after the `i.e.' so
%that the reader can `visualize' what that means? I also see the inverse, in
%which some sequential execution (as oppose to concurrent) can be asynchronous,
%as for example when two tasks are run within a single thread by the OS, but one
%does not depend on the other, i.e., one does not have to wait for the other to
%complete to start/stop. E.g., given 3 tasks and 1 thread, they are synchronous
%when 2 as to wait for 1 to finish to start; asynchronous when 2 can start
%independent of the state of 1---1 has started, 1 has completed, 1 is still
%running.}
% }
%
\subsection{Task Execution Time and Masking \FIXME{Is this a condition. I think it is more of a results I suggest we add a new section for this as benefits of WLA}}
\label{ssec:cond-ttx}

\mtnote{I think the flow might be: 1. we (formally?) define asynchronous
execution of heterogeneous workflow's tasks; 2. Once we know what asynchronous
execution is, we (formally?) explore the effects that asynchronous execution has
on commonly used metrics of workflow execution efficiency, i.e., makespan and
resource utilization; 3. We show that those effects depend on task and graph
properties, i.e., asynchronicy alone is not guarantee of better resource
utilization and/or makespan.}
\ozgurnote{That sounds good to me I will try a complete rewrite of theis entire section  with your suggestion as next section.
We can decide which one to keep}
\ozgurnote{I didn't se much to change I mainly rewrite the begining of the main section and changed the names of section and sub section
Could you please check and let me know what you think?
}

A primary motivation for asynchronous task execution is to improve resource
utilization which is directly correlated with task throughput. However, examples
have already been given that show how the introduction of asynchronicity does
not guarantee increased task throughput, specifically when the majority of
upstream tasks (ancestors) dominate resource use. On the other hand, when
resource requirements endow a workflow with a $\doares > 0$ and it is possible
to exploit TX, the overall workflow TTX can be reduced; in other words, one can
achieve higher task throughput.

Leveraging TX can afford \textit{masking}, a technique wherein longer running
tasks effectively `hide' contributions from shorter running tasks' a workflow's
TTX. To illustrate masking, consider the workflow DG of
Fig.~\ref{sfig:graph-doa1} for which $\doadep = 1$. Assume the allocated
resources are such that once $T_0$ completes, the chains $\{T_1, T_3, T_5\}$ and
$\{T_2, T_4\}$ can execute asynchronously; then $\doares = \doadep = 1$. For
concreteness, further assume the following TTX assignments:
\begin{equation*}
    t_0 = 500\text{s},~t_1 = t_2 = 1000\text{s},~2t_3 = 2t_5 = t_4 = 4000\text{s}.
\end{equation*}

To demonstrate the utility of masking, we begin with a purely sequential
workflow using the Pipeline/Stage/Task (PST)
model~\cite{balasubramanian2018harnessing}, where the DG represents a pipeline,
each rank corresponds to a stage, and each task set to tasks. In the sequential
model, the TTX is given by,
%
%\begin{align}
\begin{equation}
    \tseq = \sum_i t_i + C, \label{eqn:tseq}
\end{equation}
%\end{align}
%
% \TODO{
where $i$ represents $i$th stage and $t$ represents TX of given stage,
% }
and $C$ is a constant representing the workflow management system's overheads
such as communications. In general, $C$ is negligible with task execution times
$O(10)$ minutes and larger. As such, we disregard small overheads in future
calculations but consider them in later analyses. Plugging into
Eqn.~\ref{eqn:tseq} the above assigned TX values, the sequential TTX is
$t^{\text{Seq}} = 7500\text{s}$.

We now demonstrate how the workflow TTX can be significantly reduced by
exploiting the conditions for asynchronicity and the parameters of the workflow;
specifically here, $\text{WLA} = \min(\doadep, \doares) = 1$ and the TX
assignments
% \TODO{
are the same as above.
% }.
First, the WLA enables asynchronous execution of the chains $H_1 \equiv \{T_1,
T_3, T_5\}$ and $H_2 \equiv \{T_2, T_4\}$. Second, the TX assignments lead to
masking such that the contribution from task set $T_5$ to the workflow TTX is
hidden by the execution of task set $T_4$ since $t_4 = t_3 + t_5$ and the
corresponding task sets now execute asynchronously. In general, the asynchronous
TTX for an asynchronous workflow is given by,
%
% \FIXME{OLD one to delete}
% \begin{align}
%     \label{eqn:tasync}
%     \tasync &= \sum_{i < j} t_i + \max[t_{H_j}]  \\
%             &\leq \tseq, \nonumber
% \end{align}
%
% \FIXME{New one}
\begin{align}
% \begin{equation}
    \label{eqn:tasync}
    \tasync &= \sum_{i} t_i + \max[tt_{H_j}] + C \\
            &\leq \tseq, \nonumber
% \end{equation}
\end{align}
%
% \TODO{
where $t_i$ represents the sequential task sets and $tt_{H_j}$ represents the
TTX of each independent branch.
% }
\begin{align}
%\begin{equation}
    \label{eqn:tth}
    tt_{H_j}&= \sum_{j} t_j  \\
            &\leq \tseq, \nonumber
%\end{equation}
\end{align}
%
% \DELETE{where the sum is over the sequential task sets and $j$ corresponds to
% the task set with the smallest index within the rank where one more
% asynchronicity-permitting forks occur (in this case, $j=1$).
% }
We have equality if and only if $t_{H_j} = t_{H_k}~\forall_{j,k}$. Asynchronous
execution of the workflow under discussion therefore has a TTX of $t_0 + t_{H_1}
= 5500\text{s}$. We define the relative improvement as,
%
\begin{align}
%\begin{equation}
    I &\equiv 1 - \frac{\tasync}{\tseq},
    \label{eqn:relimp}
%\end{equation}
\end{align}
%
for which, in this example, gives roughly a 26\% reduction compared to the
sequential execution. This example makes clear the potential gains when a
workflow is designed to leverage WLA as well as TX masking.


==> submissions/JSSPP_reviews.tex <==
%!TEX root = main.tex

\subsection{Summary}

\paragraph{Reviewer 1: Strong Accept}
\begin{itemize}
    \item Additional sharing of the synthetic workflows and all code associated with the experiments as supplemental materials on Zenodo or similar archiving services.
        \begin{itemize}
            \item Ozgur: I will try to find the code that has been used to run the experiments
            \item Ozgur:  I put the code from Vince (v4) under the code  and  we can move it to GitHub
        \end{itemize}
    \item Acronyms need to explain (One nitpick: the paper mentions HPC and ML in the abstract without expansion. Later, other acronyms are used, such as GPU and MPI. Not all readers at all points in time would immediately know what these mean, so they should be expanded on the first mention.)
        \begin{itemize}
            \item Ozgur: I will check the entire paper to add explanations/citations.
            \item Ozgur: I think I fixed all of them. 
        \end{itemize}
\end{itemize}


\paragraph{Reviewer 2:  Reject}
\begin{itemize}
    \item Contributions are not clear
    \item Asynchronous implementation of DeepDriveMD isn't detailed enough
        ]\begin{itemize}
            \item Ozgur: I tried to address this in \ref{ssec:perf-ddmd}
        \end{itemize}
    \item Synthetic workload that neglects data movement and other aspects specific to real-world, ML-driven workflows. 
        \begin{itemize}
            \item Ozgur: While I agree to this comments I think (1) we do show a non-syntactic workflow with ExaLearn and (2) I think this could be a future work and I addressed this as a future work in Section \ref{sec:perf}.
        \end{itemize}
    \item Section 3 is verbose and repeats previous points
    \item The explanations of asynchronous communication and asynchronous staging is probably not helpful
    \item Notation used in Figure 1 is not clearly explained in the text
        \begin{itemize}
            \item Ozgur: I think this would be good to add since we do not have any page limit anymore.
            \item Ozgur: I added small explanation to the figures caption.
        \end{itemize}
    \item The terms TX and TTX should be defined
        \begin{itemize}
            \item Ozgur: I will check the entire paper to add explanations.
            \item Ozgur: I checked and both TTX and TX was already defined
        \end{itemize}
\end{itemize}

\paragraph{Reviewer 3: Strong Accept}
\begin{itemize}
    \item Future expansion of this research could focus on more tangible variables in the experiment, such as a scheduler or hardware variations
        \begin{itemize}
            \item Ozgur: I think it is worth to think about but I don't think we need to add any text to this paper about this. 
        \end{itemize}
    \item I would have preferred linear graphs for some of the execution time outcomes.
        \begin{itemize}
            \item Ozgur: I am not sure if Linear graphs would be better than what we currently have. Also sadly I don't have the data to redo the graphs.
        \end{itemize}
\end{itemize}


\subsection{REVIEW 1}


SCORE: 3 (strong accept)

This paper looks at an AI-driven HPC workflow (DeepDriveMD) to model the degree of asynchronicity between training/simulation and inference tasks. The former use MPI and run for hours and the latter are short and run in Python. The paper performs an experimental evaluation of the asynchronous execution and compares it to an analytical model.

This use case of large-scale computers is rapidly emerging in importance. The methodology in this paper appears sound, the experimental evaluation convincing, and the topic is timely and well within the scope of JSSPP. I would love to see this paper published in JSSPP. I think the submission would be significantly strengthened by the additional sharing of the synthetic workflows and all code associated with the experiments as supplemental materials on Zenodo or similar archiving services.


One nitpick: the paper mentions HPC and ML in the abstract without expansion. Later, other acronyms are used such as GPU and MPI. Not all readers at all points in time would immediately know what these mean, so they should be expanded on the first mention.



\subsection{REVIEW 2}

SCORE: -2 (reject)

The paper discusses asynchronous task execution of ML-driven workflows and compares the performance of sequential and asynchronous workflow executions using synthetic workloads. 

\paragraph{Strength}
The paper addresses an interesting problem and is easy to understand.

\paragraph{Weaknesses}
The research contribution of the paper is not clear. While the paper claims four contributions, it is difficult to see how these claims are justified. Specifically, the asynchronous implementation of the DeepDriveMD framework is not presented in sufficient detail. The model of asynchronous behavior in section 5 relies on simple, well-known principles in parallel computing (e.g., Brent's theorem) and cannot be seen as a contribution in itself. The performance evaluation confirms the anticipated advantages of asynchronous execution over sequential execution. Moreover, the evaluation uses a synthetic workload that neglects data movement and other aspects specific to real-world, ML-driven workflows.

The presentation of the paper could be improved. Section 3 is verbose and repeats previous points. The explanations of asynchronous communication and asynchronous staging is probably not helpful, and the notation used in Figure 1 is not clearly explained in the text. The terms TX and TTX should be defined.



\subsection{REVIEW 3}

SCORE: 3 (strong accept)

I really enjoyed reading this paper, it explored multiple aspects of the relationship between ML simulations and scheduler execution. It was well written and well structured and explained in context numerous experimental design choices and variations.

The authors explained in detail multiple approached that alter the outcomes of experimentation. Of particular interest are the role of deep neural networks, task dependency graphs and the varying impacts of control and data flows. They explain concepts seminal to this space such as the availability of concurrency and the reality of heterogeneous task design. The authors provide good insight for the researcher or practitioner looking to understand both scheduling and optimisation techniques such as attribute selection and asynchronous approaches in multiple methods (execution, communitation, data staging).

Often papers of this nature are limited to academic scale and constraints. In this case the authors chose platform sizes that were relevant to industry practitioners and provided good insights into the role of resource constraints in performance outcomes. Recommendations are given into attributes such as task time and makespan and how asynchronicity can be adapted for improved wall time. 

I was particularly enamoured of the section on abstract dependency graphs and the multiple models experienced in the heterogenous loads. These are critical to industry application of this work where multiple passes and sequential pipelines are common. Similarly the breakdown of work into simulation, aggregation, training and inference are common elements of the HPC ecosystem and show a strong understanding of the landscape. Details of the DeepDriveMD workflow are provided for the reader to understand the experimental approach, quantitative improvements given various environmental factors are provided in the conclusion. 

This paper is good and I have limited criticism of the approaches or the contextual detail provided, especially given the range of tasks and graph types engaged. Future expansion of this research could focus on more tangible variables in the experiment such as scheduler or hardware variations. I would have preferred linear graphs for some of the execution time outcomes.

==> usecase.tex <==
%!TEX root = main.tex

Drug discovery is a very resource intensive process in which a clinically tested
drug may require 15 years and over 1 billion
dollars~\cite{saha2020pharmaceutical} to reach the market. Considering the
$\approx10^{68}$ possible compounds to explore to find effective drugs, there is
an immediate need for efficient computational frameworks that can enable early
stage drug discovery~\ref{bohacek1996art}.

In the context of COVID-19, the drug-discovery community needs to identify high
quality lead molecules that have the potential to inhibit the virus life
cycle~\ref{parks2020discover}. That poses a grand challenge to screen tens of
billions of small molecules against the SARS-CoV-2 proteome. To match that
challenge, no single algorithm or method can achieve the necessary accuracy with
required efficiency. IMPECCABLE overcomes that limitation by bringing together
multiple algorithms into an unified computational campaign.

Fig.~\ref{fig:impeccable} shows IMPECCABLE's design, composed of an iterative
loop initiated with ML predictions (ML1), followed by three stages of data
processing (S1, S2, S3). IMPECCABLE centers on the use of ML techniques (ML1
and S2) interfaced with physics-based computational methods to estimate docking
poses of compounds that are promising leads for a given protein target (S1) and
binding free-energy computations (S3).

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/impeccable-gb20-level-1-v3}
    \vspace{-3mm}
    \caption{IMPECCABLE is a virtual drug discovery pipeline. The constituent
    components are deep-learning based surrogate model for docking (ML1),
    Autodock-GPU (S1), coarse and fine-grained binding free energies (S3-CG and
    S3-FG) and S2 (DeepDriveMD).}\label{fig:impeccable}
   \vspace{-0.1in}
  \end{figure}

In Refs.~\cite{saadi2021impeccable,bhati2021pandemic,brace2021achieving}, we
implemented IMPECCABLE with diverse proof of concept prototypes, using
DeepDriveMD to couple ML and molecular dynamic simulations. Each prototype was
tailored to a specific campaign, reaching high-levels of scalability compared to
other approaches. The performance characterization of those prototypes
established that, when feasible, asynchronous execution of ML and simulation
tasks can improve both resource utilization and task throughput. Nonetheless,
the implementation of such an execution model depends on specific capabilities
of the task utilized and cannot be applied to all the type of tasks executed via
DeepDriveMD as part of IMPECCABLE.

IMPECCABLE requires a general purpose approach to asynchronous task execution in
DeepDriveMD. That approach does not depend on the specific implementation of
each task, remains agnostic towards the communication and data capabilities of
each task and makes no assumptions about streaming capabilities. DeepDriveMD
must account for tasks that have to be executed sequentially, those that can
concurrently execute and communicate or exchanging data, and those that have no
relationship and can be executed either concurrently or sequentially.
Precondition to such a general-purpose design is to understand both conceptually
and experimentally how asynchronous execution can affect the performance of a
given workflow composed of diverse types of tasks.
